Convergence guarantee for the sparse monotone single index model

We consider a high-dimensional monotone single index model (hdSIM), which is a semiparametric extension of a high-dimensional generalize linear model (hdGLM), where the link function is unknown, but constrained with monotone and non-decreasing shape. We develop a scalable projection-based iterative approach, the "Sparse Orthogonal Descent Single-Index Model" (SOD-SIM), which alternates between sparse-thresholded orthogonalized "gradient-like" steps and isotonic regression steps to recover the coefficient vector. Our main contribution is that we provide finite sample estimation bounds for both the coefficient vector and the link function in high-dimensional settings under very mild assumptions on the design matrix $\mathbf{X}$, the error term $\epsilon$, and their dependence. The convergence rate for the link function matched the low-dimensional isotonic regression minimax rate up to some poly-log terms ($n^{-1/3}$). The convergence rate for the coefficients is also $n^{-1/3}$ up to some poly-log terms. This method can be applied to many real data problems, including GLMs with misspecified link, classification with mislabeled data, and classification with positive-unlabeled (PU) data. We study the performance of this method via both numerical studies and also an application on a rocker protein sequence data.

==> rocker.tex <==
\section{Application to rocker data}	
In this section, we study an application of our algorithm to a rocker protein sequence data. The rocker data is a kind of PU data, which contain functional sequences and sequences with unknown functionality. 

To give some biological context to this dataset, Rocker is a \emph{de novo} designed protein which recreates the biological function of substrate transportation \citep{Joh2014-xy}. A functional protein of this kind successfully transports ions across cell membranes. To study how a mutation at each site affects the membrane transport ability of proteins, mutations are introduced to the original Rocker sequence (wild-type) by double site saturation mutagenesis. %Mutated sequences differ by at most two sites from the wild-type sequence.  
Mutated sequences are screened by fluorescence-activated cell sorting (FACS), which sort out \emph{functional} protein variants. Due to an experimental challenge of obtaining negative sequences, an additional set of sequences are obtained from the initial library whose associated functionality is unknown. Therefore, the resulting data set is a Positive-Unlabeled (PU) dataset, because the first set consists of functional sequence variants and the second set consists unlabeled examples.

A sequence consists of 25 positions which takes one of the $21$ discrete values which correspond to 20 amino acid letter codes plus an additional letter for the alignment gap. Each sequence contains at most two mutations. The data consists of $n_\ell = 703030$ functional (positive label) and $n_u = 1287155$ unlabeled sequences. To compare different algorithms reliably, we split the data into 10 subsets, and use a half of each split for training and remaining half for testing. Each training dataset contains 35K labeled and 64K unlabeled examples on average.  We generate features with main (site-wise) and pairwise (interaction between two sites) effects using one-hot encoding of the sequences. Removing columns with zero counts, we obtain 27K features on average, where 490 of the generated features correspond to the main effects. We take the amino acid levels in the WT sequence as the baseline levels to generate a sparse design matrix $\mathbf{X} \in \mathbb{R}^{n\times p}$ where $(n,p) \approx$ (100K, 27K). The number of unique sequences is around 26K (i.e., rank of row space of $\mathbf{X}\approx$ 26K), which makes the problem high-dimensional. The response vector $\mathbf{Y}\in \mathbb{R}^{n}$ represents whether each sequence $i$ is labeled ($\mathbf{Y}_i =1$) or unlabeled ($\mathbf{Y}_i =0$). %Finally, grouping sequences into their unique levels, we obtained a sparse design matrix $\mathbf{X} \in \mathbb{R}^{n \times p}$, a response $\mathbf{Y} \in \mathbb{R}^{n\times 1}$, and a diagonal weight matrix $\mathbf{W} \in \mathbb{R}^{n\times n}$, where each $\mathbf{Y}_i \in \{0,1\}$ represents whether the $i$th sequence is labeled ($\mathbf{Y}_i =1$) or unlabeled ($\mathbf{Y}_i =0$), and a diagonal element of the weight matrix $\mathbf{W}_{ii}$ corresponds to a count of the 


We applied four methods to each train dataset which we denote as follows:
\begin{itemize}
	\item hdSIM: our algorithm
	\item sparseLR: the logistic regression with $\ell_1$-penalty
	\item PV1: the proposed method in \cite{Plan2013-ew}. We solve the following objective:
$$ \hat{u}^{PV1}  \in \arg \max_{u \in K(s)} \langle y, \mathbf{X} u\rangle$$
where $K(s)$ is a $s$-approximate sparse set, defined as $K(s) := \{x\in \mathbb{R} : \|x\|_2 \leq 1,  \|x\|_1\leq \sqrt{s}\}$
    
	\item PV2: the proposed method in \cite{Plan2016-cz}. 
$$ \hat{u}^{PV2}  \in \arg \min_{u \in K(s)} \|y-\mathbf{X} u \|_2. $$
\end{itemize}


We used a \textbf{glmnet} package to solve the logistic regression objective with $\ell_1$-penalty. To solve objectives in PV1 and PV2, we implemented the projected gradient methods, where we iteratively projected the gradients onto the intersection of $\ell_1$ and $\ell_2$ balls. We used the Dykstra's projection algorithm to obtain the projection onto the intersection of the two balls \citep{Boyle1986-us}. Note both objectives in PV1 and PV2 are convex, and therefore the projected gradient descent algorithm guarantees to find a global minimum. For PV1 and PV2, we input the standardized $\mathbf{X}$ where each column is centered and scaled. Since sparseLR, PV1, and PV2 are convex problems, we run until the algorithms the models converge. For hdSIM, we run the algorithm until changes of estimated parameters is small ($< 0.0005$) or the iteration number $t$ reaches the pre-defined maximum number of iterations ($\leq 500$). In addition, PV1 and PV2 methods do not provide estimates of the link function. We run an isotonic regression after obtaining $\hat{u}^{PV1}$ and $\hat{u}^{PV2}$ to estimate the link function, and used such estimates to perform downstream prediction tasks. 

We used four metrics (Accuracy, F1 score, Brier Score, and AUC value) to evaluate predictive performance of the four methods. Accuracy is the proportion of correctly classified examples. F1 score is the harmonic mean of the precision and recall, whose value lies between 0 and 1. Higher number corresponds to a better performance. Brier Score is an average squared $\ell_2$ loss, i.e., Brier Score := $\frac{1}{n_{test}} \sum_{i=1}^{n_{test}} (y_i - \hat{y}_i)^2$, and therefore, lower numbers correspond to better performances. AUC measures the area under the ROC curve. The perfect classification corresponds to the AUC value of 1, and a random classification corresponds to 0.5. For the choice of hyperparameters ($s$ for hdSIM, PV1, and PV2, and $\lambda$ for the $\ell_1$ logistic regression), we use a grid of 100 working sparsity $s$ values from 1 to $p$, interpolated in a square root scale, and a grid of 100 lambda values obtained from the \textbf{glmnet} package by default. We picked the hyperparameters that gave the best results for the most of the metrics on the test datasets. 

Figure \ref{fig:fig1} demonstrates the empirical performances of the four methods. hdSIM performed the best in all metrics on average. The predictive performance of the sparse logistic regression was slightly worse than the hdSIM. It is likely due to the mis-specification error, since we are forcing the link function to be a sigmoid function. Both PV1 and PV2 seem to suffer from the deviation $\mathbf{X}$ from the Gaussian design; however, PV2 seems to be more robust to such deviation.

\begin{figure}[ht]
\centering
\includegraphics[width=.7\linewidth]{empComp}	
\caption{Average accuracy rates, F1 scores, 1-Brier Score, and AUC values of the four methods on 10 test datasets. Higher values correspond to better performance in all four plots. The error bars represent one standard error.}
\end{figure}\label{fig:fig1}

